Revisiting Oxford and Paris: Large-Scale Image Retrieval Benchmarking

In this paper we address issues with image retrieval benchmarking on standard and popular Oxford 5k and Paris 6k datasets. In particular, annotation errors, the size of the dataset, and the level of challenge are addressed: new annotation for both datasets is created with an extra attention to the reliability of the ground truth. Three new protocols of varying difficulty are introduced. The protocols allow fair comparison between different methods, including those using a dataset pre-processing stage. For each dataset, 15 new challenging queries are introduced. Finally, a new set of 1M hard, semi-automatically cleaned distractors is selected. An extensive comparison of the state-of-the-art methods is performed on the new benchmark. Different types of methods are evaluated, ranging from local-feature-based to modern CNN based methods. The best results are achieved by taking the best of the two worlds. Most importantly, image retrieval appears far from being solved.

==> fig/data/ap_hist_q1.tex <==
\pgfplotstableread{
q vlad asmksp delfasmksp hqesp delfhqesp vggoffrmac resoffgem resftgem resftgemdfs resftgemspdfs
1 0.10 0.31 0.43 0.72 0.59 0.20 0.11 0.28 0.75 0.81
}{\aphistoxf}
\pgfplotstableread{
q vlad asmksp delfasmksp hqesp delfhqesp vggoffrmac resoffgem resftgem resftgemdfs resftgemspdfs
1 0.05 0.32 0.61 0.44 0.46 0.41 0.53 0.49 0.81 0.81
}{\aphistpar}


==> fig/data/ap_hist_q10.tex <==
\pgfplotstableread{
q vlad asmksp delfasmksp hqesp delfhqesp vggoffrmac resoffgem resftgem resftgemdfs resftgemspdfs
10 0.21 0.34 0.34 0.55 0.47 0.22 0.20 0.31 0.64 0.63
}{\aphistoxf}
\pgfplotstableread{
q vlad asmksp delfasmksp hqesp delfhqesp vggoffrmac resoffgem resftgem resftgemdfs resftgemspdfs
10 0.04 0.19 0.52 0.32 0.54 0.25 0.37 0.43 0.80 0.82
}{\aphistpar}


==> fig/data/ap_hist_q11.tex <==
\pgfplotstableread{
q vlad asmksp delfasmksp hqesp delfhqesp vggoffrmac resoffgem resftgem resftgemdfs resftgemspdfs
11 0.30 0.59 0.60 0.39 0.72 0.17 0.07 0.43 0.49 0.72
}{\aphistoxf}
\pgfplotstableread{
q vlad asmksp delfasmksp hqesp delfhqesp vggoffrmac resoffgem resftgem resftgemdfs resftgemspdfs
11 0.15 0.34 0.67 0.57 0.71 0.44 0.51 0.54 0.74 0.75
}{\aphistpar}


==> fig/data/ap_hist_q12.tex <==
\pgfplotstableread{
q vlad asmksp delfasmksp hqesp delfhqesp vggoffrmac resoffgem resftgem resftgemdfs resftgemspdfs
12 0.13 0.50 0.51 0.50 0.51 0.00 0.08 0.50 0.08 0.50
}{\aphistoxf}
\pgfplotstableread{
q vlad asmksp delfasmksp hqesp delfhqesp vggoffrmac resoffgem resftgem resftgemdfs resftgemspdfs
12 0.18 0.39 0.61 0.58 0.68 0.47 0.47 0.55 0.74 0.74
}{\aphistpar}


==> fig/data/ap_hist_q13.tex <==
\pgfplotstableread{
q vlad asmksp delfasmksp hqesp delfhqesp vggoffrmac resoffgem resftgem resftgemdfs resftgemspdfs
13 0.00 0.01 0.40 0.00 0.41 0.00 0.00 0.41 0.60 0.00
}{\aphistoxf}
\pgfplotstableread{
q vlad asmksp delfasmksp hqesp delfhqesp vggoffrmac resoffgem resftgem resftgemdfs resftgemspdfs
13 0.27 0.57 0.68 0.63 0.70 0.46 0.50 0.57 0.74 0.75
}{\aphistpar}


==> fig/data/ap_hist_q14.tex <==
\pgfplotstableread{
q vlad asmksp delfasmksp hqesp delfhqesp vggoffrmac resoffgem resftgem resftgemdfs resftgemspdfs
14 0.08 0.37 0.55 0.50 0.55 0.01 0.17 0.53 0.76 0.77
}{\aphistoxf}
\pgfplotstableread{
q vlad asmksp delfasmksp hqesp delfhqesp vggoffrmac resoffgem resftgem resftgemdfs resftgemspdfs
14 0.16 0.48 0.72 0.63 0.74 0.47 0.53 0.55 0.76 0.77
}{\aphistpar}


==> fig/data/ap_hist_q15.tex <==
\pgfplotstableread{
q vlad asmksp delfasmksp hqesp delfhqesp vggoffrmac resoffgem resftgem resftgemdfs resftgemspdfs
15 0.07 0.52 0.57 0.74 0.61 0.01 0.02 0.58 0.67 0.73
}{\aphistoxf}
\pgfplotstableread{
q vlad asmksp delfasmksp hqesp delfhqesp vggoffrmac resoffgem resftgem resftgemdfs resftgemspdfs
15 0.22 0.46 0.67 0.60 0.69 0.46 0.51 0.55 0.74 0.74
}{\aphistpar}


==> fig/data/ap_hist_q16.tex <==
\pgfplotstableread{
q vlad asmksp delfasmksp hqesp delfhqesp vggoffrmac resoffgem resftgem resftgemdfs resftgemspdfs
16 0.00 0.33 0.68 0.00 0.66 0.05 0.07 0.10 0.56 0.73
}{\aphistoxf}
\pgfplotstableread{
q vlad asmksp delfasmksp hqesp delfhqesp vggoffrmac resoffgem resftgem resftgemdfs resftgemspdfs
16 0.14 0.53 0.73 0.65 0.84 0.49 0.62 0.59 0.97 0.97
}{\aphistpar}


==> fig/data/ap_hist_q17.tex <==
\pgfplotstableread{
q vlad asmksp delfasmksp hqesp delfhqesp vggoffrmac resoffgem resftgem resftgemdfs resftgemspdfs
17 0.06 0.33 0.58 0.13 0.64 0.07 0.12 0.36 0.68 0.73
}{\aphistoxf}
\pgfplotstableread{
q vlad asmksp delfasmksp hqesp delfhqesp vggoffrmac resoffgem resftgem resftgemdfs resftgemspdfs
17 0.13 0.27 0.68 0.11 0.72 0.45 0.63 0.65 0.97 0.97
}{\aphistpar}


==> fig/data/ap_hist_q18.tex <==
\pgfplotstableread{
q vlad asmksp delfasmksp hqesp delfhqesp vggoffrmac resoffgem resftgem resftgemdfs resftgemspdfs
18 0.12 0.33 0.58 0.23 0.58 0.10 0.05 0.43 0.76 0.76
}{\aphistoxf}
\pgfplotstableread{
q vlad asmksp delfasmksp hqesp delfhqesp vggoffrmac resoffgem resftgem resftgemdfs resftgemspdfs
18 0.05 0.21 0.52 0.08 0.71 0.10 0.54 0.39 0.96 0.96
}{\aphistpar}


==> fig/data/ap_hist_q19.tex <==
\pgfplotstableread{
q vlad asmksp delfasmksp hqesp delfhqesp vggoffrmac resoffgem resftgem resftgemdfs resftgemspdfs
19 0.00 0.44 0.39 0.56 0.77 0.01 0.00 0.05 0.00 0.78
}{\aphistoxf}
\pgfplotstableread{
q vlad asmksp delfasmksp hqesp delfhqesp vggoffrmac resoffgem resftgem resftgemdfs resftgemspdfs
19 0.14 0.29 0.64 0.11 0.79 0.28 0.60 0.39 0.96 0.96
}{\aphistpar}


==> fig/data/ap_hist_q2.tex <==
\pgfplotstableread{
q vlad asmksp delfasmksp hqesp delfhqesp vggoffrmac resoffgem resftgem resftgemdfs resftgemspdfs
2 0.21 0.48 0.38 0.52 0.63 0.24 0.22 0.28 0.75 0.85
}{\aphistoxf}
\pgfplotstableread{
q vlad asmksp delfasmksp hqesp delfhqesp vggoffrmac resoffgem resftgem resftgemdfs resftgemspdfs
2 0.03 0.22 0.61 0.38 0.70 0.46 0.61 0.58 0.81 0.81
}{\aphistpar}


==> fig/data/ap_hist_q20.tex <==
\pgfplotstableread{
q vlad asmksp delfasmksp hqesp delfhqesp vggoffrmac resoffgem resftgem resftgemdfs resftgemspdfs
20 0.00 0.40 0.67 0.52 0.77 0.01 0.01 0.13 0.00 0.75
}{\aphistoxf}
\pgfplotstableread{
q vlad asmksp delfasmksp hqesp delfhqesp vggoffrmac resoffgem resftgem resftgemdfs resftgemspdfs
20 0.05 0.32 0.53 0.29 0.73 0.41 0.53 0.54 0.97 0.97
}{\aphistpar}


==> fig/data/ap_hist_q21.tex <==
\pgfplotstableread{
q vlad asmksp delfasmksp hqesp delfhqesp vggoffrmac resoffgem resftgem resftgemdfs resftgemspdfs
21 0.35 0.65 0.81 0.67 0.87 0.44 0.61 0.68 0.75 0.76
}{\aphistoxf}
\pgfplotstableread{
q vlad asmksp delfasmksp hqesp delfhqesp vggoffrmac resoffgem resftgem resftgemdfs resftgemspdfs
21 0.02 0.22 0.51 0.39 0.70 0.57 0.44 0.58 0.97 0.97
}{\aphistpar}


==> fig/data/ap_hist_q22.tex <==
\pgfplotstableread{
q vlad asmksp delfasmksp hqesp delfhqesp vggoffrmac resoffgem resftgem resftgemdfs resftgemspdfs
22 0.23 0.63 0.82 0.69 0.88 0.40 0.59 0.71 0.75 0.75
}{\aphistoxf}
\pgfplotstableread{
q vlad asmksp delfasmksp hqesp delfhqesp vggoffrmac resoffgem resftgem resftgemdfs resftgemspdfs
22 0.03 0.25 0.57 0.19 0.68 0.67 0.66 0.73 0.97 0.97
}{\aphistpar}


==> fig/data/ap_hist_q23.tex <==
\pgfplotstableread{
q vlad asmksp delfasmksp hqesp delfhqesp vggoffrmac resoffgem resftgem resftgemdfs resftgemspdfs
23 0.02 0.38 0.74 0.65 0.86 0.44 0.56 0.67 0.75 0.75
}{\aphistoxf}
\pgfplotstableread{
q vlad asmksp delfasmksp hqesp delfhqesp vggoffrmac resoffgem resftgem resftgemdfs resftgemspdfs
23 0.01 0.24 0.70 0.34 0.81 0.55 0.68 0.87 0.97 0.97
}{\aphistpar}


==> fig/data/ap_hist_q24.tex <==
\pgfplotstableread{
q vlad asmksp delfasmksp hqesp delfhqesp vggoffrmac resoffgem resftgem resftgemdfs resftgemspdfs
24 0.22 0.67 0.84 0.68 0.88 0.43 0.59 0.72 0.75 0.75
}{\aphistoxf}
\pgfplotstableread{
q vlad asmksp delfasmksp hqesp delfhqesp vggoffrmac resoffgem resftgem resftgemdfs resftgemspdfs
24 0.03 0.34 0.56 0.46 0.67 0.60 0.69 0.75 0.97 0.97
}{\aphistpar}


==> fig/data/ap_hist_q25.tex <==
\pgfplotstableread{
q vlad asmksp delfasmksp hqesp delfhqesp vggoffrmac resoffgem resftgem resftgemdfs resftgemspdfs
25 0.00 0.26 0.47 0.37 0.70 0.01 0.18 0.36 0.50 0.54
}{\aphistoxf}
\pgfplotstableread{
q vlad asmksp delfasmksp hqesp delfhqesp vggoffrmac resoffgem resftgem resftgemdfs resftgemspdfs
25 0.09 0.41 0.58 0.46 0.77 0.53 0.61 0.60 0.97 0.97
}{\aphistpar}


==> fig/data/ap_hist_q26.tex <==
\pgfplotstableread{
q vlad asmksp delfasmksp hqesp delfhqesp vggoffrmac resoffgem resftgem resftgemdfs resftgemspdfs
26 0.08 0.39 0.31 0.37 0.28 0.17 0.13 0.36 0.33 0.47
}{\aphistoxf}
\pgfplotstableread{
q vlad asmksp delfasmksp hqesp delfhqesp vggoffrmac resoffgem resftgem resftgemdfs resftgemspdfs
26 0.23 0.51 0.45 0.28 0.41 0.28 0.37 0.41 0.93 0.94
}{\aphistpar}


==> fig/data/ap_hist_q27.tex <==
\pgfplotstableread{
q vlad asmksp delfasmksp hqesp delfhqesp vggoffrmac resoffgem resftgem resftgemdfs resftgemspdfs
27 0.00 0.08 0.01 0.00 0.01 0.00 0.00 0.16 0.16 0.03
}{\aphistoxf}
\pgfplotstableread{
q vlad asmksp delfasmksp hqesp delfhqesp vggoffrmac resoffgem resftgem resftgemdfs resftgemspdfs
27 0.00 0.85 0.76 0.64 0.83 0.26 0.41 0.42 0.92 0.96
}{\aphistpar}


==> fig/data/ap_hist_q28.tex <==
\pgfplotstableread{
q vlad asmksp delfasmksp hqesp delfhqesp vggoffrmac resoffgem resftgem resftgemdfs resftgemspdfs
28 0.01 0.39 0.18 0.36 0.08 0.10 0.02 0.16 0.17 0.47
}{\aphistoxf}
\pgfplotstableread{
q vlad asmksp delfasmksp hqesp delfhqesp vggoffrmac resoffgem resftgem resftgemdfs resftgemspdfs
28 0.20 0.45 0.56 0.43 0.76 0.35 0.45 0.43 0.92 0.92
}{\aphistpar}


==> fig/data/ap_hist_q29.tex <==
\pgfplotstableread{
q vlad asmksp delfasmksp hqesp delfhqesp vggoffrmac resoffgem resftgem resftgemdfs resftgemspdfs
29 0.00 0.23 0.20 0.14 0.03 0.18 0.08 0.29 0.23 0.34
}{\aphistoxf}
\pgfplotstableread{
q vlad asmksp delfasmksp hqesp delfhqesp vggoffrmac resoffgem resftgem resftgemdfs resftgemspdfs
29 0.18 0.32 0.41 0.16 0.29 0.28 0.30 0.31 0.93 0.89
}{\aphistpar}


==> fig/data/ap_hist_q3.tex <==
\pgfplotstableread{
q vlad asmksp delfasmksp hqesp delfhqesp vggoffrmac resoffgem resftgem resftgemdfs resftgemspdfs
3 0.21 0.47 0.44 0.57 0.67 0.24 0.27 0.29 0.75 0.88
}{\aphistoxf}
\pgfplotstableread{
q vlad asmksp delfasmksp hqesp delfhqesp vggoffrmac resoffgem resftgem resftgemdfs resftgemspdfs
3 0.08 0.31 0.61 0.43 0.68 0.41 0.53 0.49 0.81 0.80
}{\aphistpar}


==> fig/data/ap_hist_q30.tex <==
\pgfplotstableread{
q vlad asmksp delfasmksp hqesp delfhqesp vggoffrmac resoffgem resftgem resftgemdfs resftgemspdfs
30 0.00 0.36 0.34 0.33 0.33 0.02 0.09 0.31 0.33 0.46
}{\aphistoxf}
\pgfplotstableread{
q vlad asmksp delfasmksp hqesp delfhqesp vggoffrmac resoffgem resftgem resftgemdfs resftgemspdfs
30 0.19 0.43 0.43 0.21 0.34 0.26 0.36 0.37 0.93 0.92
}{\aphistpar}


==> fig/data/ap_hist_q31.tex <==
\pgfplotstableread{
q vlad asmksp delfasmksp hqesp delfhqesp vggoffrmac resoffgem resftgem resftgemdfs resftgemspdfs
31 0.58 0.86 0.77 0.95 0.81 0.68 0.57 0.78 0.89 0.92
}{\aphistoxf}
\pgfplotstableread{
q vlad asmksp delfasmksp hqesp delfhqesp vggoffrmac resoffgem resftgem resftgemdfs resftgemspdfs
31 0.44 0.63 0.65 0.77 0.79 0.48 0.45 0.63 0.86 0.87
}{\aphistpar}


==> fig/data/ap_hist_q32.tex <==
\pgfplotstableread{
q vlad asmksp delfasmksp hqesp delfhqesp vggoffrmac resoffgem resftgem resftgemdfs resftgemspdfs
32 0.38 0.73 0.79 0.77 0.83 0.66 0.58 0.75 0.89 0.90
}{\aphistoxf}
\pgfplotstableread{
q vlad asmksp delfasmksp hqesp delfhqesp vggoffrmac resoffgem resftgem resftgemdfs resftgemspdfs
32 0.49 0.71 0.74 0.78 0.80 0.47 0.49 0.67 0.86 0.88
}{\aphistpar}


==> fig/data/ap_hist_q33.tex <==
\pgfplotstableread{
q vlad asmksp delfasmksp hqesp delfhqesp vggoffrmac resoffgem resftgem resftgemdfs resftgemspdfs
33 0.23 0.83 0.67 0.94 0.80 0.56 0.53 0.71 0.89 0.91
}{\aphistoxf}
\pgfplotstableread{
q vlad asmksp delfasmksp hqesp delfhqesp vggoffrmac resoffgem resftgem resftgemdfs resftgemspdfs
33 0.39 0.66 0.74 0.78 0.80 0.44 0.45 0.62 0.86 0.87
}{\aphistpar}


==> fig/data/ap_hist_q34.tex <==
\pgfplotstableread{
q vlad asmksp delfasmksp hqesp delfhqesp vggoffrmac resoffgem resftgem resftgemdfs resftgemspdfs
34 0.45 0.86 0.77 0.94 0.81 0.61 0.56 0.73 0.89 0.91
}{\aphistoxf}
\pgfplotstableread{
q vlad asmksp delfasmksp hqesp delfhqesp vggoffrmac resoffgem resftgem resftgemdfs resftgemspdfs
34 0.51 0.75 0.74 0.79 0.80 0.48 0.48 0.64 0.86 0.88
}{\aphistpar}


==> fig/data/ap_hist_q35.tex <==
\pgfplotstableread{
q vlad asmksp delfasmksp hqesp delfhqesp vggoffrmac resoffgem resftgem resftgemdfs resftgemspdfs
35 0.46 0.88 0.82 0.94 0.86 0.63 0.56 0.77 0.89 0.92
}{\aphistoxf}
\pgfplotstableread{
q vlad asmksp delfasmksp hqesp delfhqesp vggoffrmac resoffgem resftgem resftgemdfs resftgemspdfs
35 0.27 0.56 0.64 0.75 0.77 0.18 0.40 0.59 0.86 0.87
}{\aphistpar}


==> fig/data/ap_hist_q36.tex <==
\pgfplotstableread{
q vlad asmksp delfasmksp hqesp delfhqesp vggoffrmac resoffgem resftgem resftgemdfs resftgemspdfs
36 0.50 1.00 1.00 0.16 1.00 0.59 1.00 1.00 1.00 1.00
}{\aphistoxf}
\pgfplotstableread{
q vlad asmksp delfasmksp hqesp delfhqesp vggoffrmac resoffgem resftgem resftgemdfs resftgemspdfs
36 0.56 0.69 0.79 0.77 0.84 0.33 0.35 0.49 0.87 0.88
}{\aphistpar}


==> fig/data/ap_hist_q37.tex <==
\pgfplotstableread{
q vlad asmksp delfasmksp hqesp delfhqesp vggoffrmac resoffgem resftgem resftgemdfs resftgemspdfs
37 0.51 1.00 1.00 0.79 1.00 0.53 0.63 1.00 1.00 1.00
}{\aphistoxf}
\pgfplotstableread{
q vlad asmksp delfasmksp hqesp delfhqesp vggoffrmac resoffgem resftgem resftgemdfs resftgemspdfs
37 0.52 0.70 0.76 0.74 0.80 0.48 0.53 0.62 0.87 0.87
}{\aphistpar}


==> fig/data/ap_hist_q38.tex <==
\pgfplotstableread{
q vlad asmksp delfasmksp hqesp delfhqesp vggoffrmac resoffgem resftgem resftgemdfs resftgemspdfs
38 0.50 1.00 1.00 0.79 1.00 0.54 0.63 1.00 1.00 1.00
}{\aphistoxf}
\pgfplotstableread{
q vlad asmksp delfasmksp hqesp delfhqesp vggoffrmac resoffgem resftgem resftgemdfs resftgemspdfs
38 0.43 0.63 0.74 0.74 0.79 0.38 0.51 0.45 0.87 0.87
}{\aphistpar}


==> fig/data/ap_hist_q39.tex <==
\pgfplotstableread{
q vlad asmksp delfasmksp hqesp delfhqesp vggoffrmac resoffgem resftgem resftgemdfs resftgemspdfs
39 0.50 0.50 1.00 1.00 1.00 0.13 0.52 0.79 1.00 1.00
}{\aphistoxf}
\pgfplotstableread{
q vlad asmksp delfasmksp hqesp delfhqesp vggoffrmac resoffgem resftgem resftgemdfs resftgemspdfs
39 0.44 0.65 0.76 0.69 0.79 0.42 0.48 0.53 0.87 0.87
}{\aphistpar}


==> fig/data/ap_hist_q4.tex <==
\pgfplotstableread{
q vlad asmksp delfasmksp hqesp delfhqesp vggoffrmac resoffgem resftgem resftgemdfs resftgemspdfs
4 0.18 0.68 0.74 0.74 0.83 0.18 0.29 0.54 0.86 0.88
}{\aphistoxf}
\pgfplotstableread{
q vlad asmksp delfasmksp hqesp delfhqesp vggoffrmac resoffgem resftgem resftgemdfs resftgemspdfs
4 0.09 0.13 0.56 0.04 0.65 0.41 0.53 0.57 0.81 0.79
}{\aphistpar}


==> fig/data/ap_hist_q40.tex <==
\pgfplotstableread{
q vlad asmksp delfasmksp hqesp delfhqesp vggoffrmac resoffgem resftgem resftgemdfs resftgemspdfs
40 0.50 1.00 1.00 1.00 1.00 0.50 0.53 1.00 1.00 1.00
}{\aphistoxf}
\pgfplotstableread{
q vlad asmksp delfasmksp hqesp delfhqesp vggoffrmac resoffgem resftgem resftgemdfs resftgemspdfs
40 0.58 0.72 0.78 0.79 0.83 0.45 0.56 0.60 0.87 0.88
}{\aphistpar}


==> fig/data/ap_hist_q41.tex <==
\pgfplotstableread{
q vlad asmksp delfasmksp hqesp delfhqesp vggoffrmac resoffgem resftgem resftgemdfs resftgemspdfs
41 0.00 0.07 0.35 0.18 0.52 0.05 0.09 0.27 0.60 0.65
}{\aphistoxf}
\pgfplotstableread{
q vlad asmksp delfasmksp hqesp delfhqesp vggoffrmac resoffgem resftgem resftgemdfs resftgemspdfs
41 0.27 0.53 0.68 0.41 0.69 0.76 0.79 0.76 0.94 0.94
}{\aphistpar}


==> fig/data/ap_hist_q42.tex <==
\pgfplotstableread{
q vlad asmksp delfasmksp hqesp delfhqesp vggoffrmac resoffgem resftgem resftgemdfs resftgemspdfs
42 0.00 0.14 0.45 0.33 0.61 0.09 0.15 0.50 0.63 0.63
}{\aphistoxf}
\pgfplotstableread{
q vlad asmksp delfasmksp hqesp delfhqesp vggoffrmac resoffgem resftgem resftgemdfs resftgemspdfs
42 0.31 0.52 0.62 0.43 0.70 0.73 0.81 0.75 0.94 0.94
}{\aphistpar}


==> fig/data/ap_hist_q43.tex <==
\pgfplotstableread{
q vlad asmksp delfasmksp hqesp delfhqesp vggoffrmac resoffgem resftgem resftgemdfs resftgemspdfs
43 0.01 0.19 0.43 0.32 0.53 0.11 0.11 0.37 0.61 0.61
}{\aphistoxf}
\pgfplotstableread{
q vlad asmksp delfasmksp hqesp delfhqesp vggoffrmac resoffgem resftgem resftgemdfs resftgemspdfs
43 0.44 0.60 0.68 0.48 0.72 0.75 0.72 0.78 0.94 0.94
}{\aphistpar}


==> fig/data/ap_hist_q44.tex <==
\pgfplotstableread{
q vlad asmksp delfasmksp hqesp delfhqesp vggoffrmac resoffgem resftgem resftgemdfs resftgemspdfs
44 0.00 0.01 0.31 0.02 0.54 0.09 0.05 0.37 0.67 0.60
}{\aphistoxf}
\pgfplotstableread{
q vlad asmksp delfasmksp hqesp delfhqesp vggoffrmac resoffgem resftgem resftgemdfs resftgemspdfs
44 0.41 0.68 0.62 0.63 0.70 0.65 0.57 0.75 0.94 0.94
}{\aphistpar}


==> fig/data/ap_hist_q45.tex <==
\pgfplotstableread{
q vlad asmksp delfasmksp hqesp delfhqesp vggoffrmac resoffgem resftgem resftgemdfs resftgemspdfs
45 0.04 0.16 0.37 0.24 0.52 0.06 0.14 0.28 0.59 0.57
}{\aphistoxf}
\pgfplotstableread{
q vlad asmksp delfasmksp hqesp delfhqesp vggoffrmac resoffgem resftgem resftgemdfs resftgemspdfs
45 0.47 0.64 0.57 0.38 0.44 0.73 0.71 0.78 0.94 0.94
}{\aphistpar}


==> fig/data/ap_hist_q46.tex <==
\pgfplotstableread{
q vlad asmksp delfasmksp hqesp delfhqesp vggoffrmac resoffgem resftgem resftgemdfs resftgemspdfs
46 0.00 1.00 1.00 1.00 1.00 0.13 0.50 0.79 1.00 1.00
}{\aphistoxf}
\pgfplotstableread{
q vlad asmksp delfasmksp hqesp delfhqesp vggoffrmac resoffgem resftgem resftgemdfs resftgemspdfs
46 0.23 0.60 0.77 0.78 0.79 0.62 0.64 0.70 0.92 0.92
}{\aphistpar}


==> fig/data/ap_hist_q47.tex <==
\pgfplotstableread{
q vlad asmksp delfasmksp hqesp delfhqesp vggoffrmac resoffgem resftgem resftgemdfs resftgemspdfs
47 1.00 1.00 1.00 1.00 1.00 0.50 0.50 1.00 1.00 1.00
}{\aphistoxf}
\pgfplotstableread{
q vlad asmksp delfasmksp hqesp delfhqesp vggoffrmac resoffgem resftgem resftgemdfs resftgemspdfs
47 0.38 0.66 0.77 0.79 0.80 0.66 0.65 0.75 0.92 0.92
}{\aphistpar}


==> fig/data/ap_hist_q48.tex <==
\pgfplotstableread{
q vlad asmksp delfasmksp hqesp delfhqesp vggoffrmac resoffgem resftgem resftgemdfs resftgemspdfs
48 0.71 1.00 1.00 1.00 1.00 0.13 0.50 1.00 1.00 1.00
}{\aphistoxf}
\pgfplotstableread{
q vlad asmksp delfasmksp hqesp delfhqesp vggoffrmac resoffgem resftgem resftgemdfs resftgemspdfs
48 0.50 0.74 0.74 0.79 0.79 0.60 0.57 0.68 0.92 0.92
}{\aphistpar}


==> fig/data/ap_hist_q49.tex <==
\pgfplotstableread{
q vlad asmksp delfasmksp hqesp delfhqesp vggoffrmac resoffgem resftgem resftgemdfs resftgemspdfs
49 0.17 1.00 1.00 1.00 1.00 0.50 0.08 0.79 0.60 1.00
}{\aphistoxf}
\pgfplotstableread{
q vlad asmksp delfasmksp hqesp delfhqesp vggoffrmac resoffgem resftgem resftgemdfs resftgemspdfs
49 0.39 0.68 0.77 0.77 0.79 0.65 0.61 0.72 0.92 0.92
}{\aphistpar}


==> fig/data/ap_hist_q5.tex <==
\pgfplotstableread{
q vlad asmksp delfasmksp hqesp delfhqesp vggoffrmac resoffgem resftgem resftgemdfs resftgemspdfs
5 0.16 0.49 0.50 0.59 0.63 0.20 0.20 0.25 0.75 0.83
}{\aphistoxf}
\pgfplotstableread{
q vlad asmksp delfasmksp hqesp delfhqesp vggoffrmac resoffgem resftgem resftgemdfs resftgemspdfs
5 0.03 0.25 0.60 0.38 0.71 0.49 0.57 0.57 0.81 0.81
}{\aphistpar}


==> fig/data/ap_hist_q50.tex <==
\pgfplotstableread{
q vlad asmksp delfasmksp hqesp delfhqesp vggoffrmac resoffgem resftgem resftgemdfs resftgemspdfs
50 0.63 1.00 1.00 1.00 1.00 0.50 0.50 1.00 1.00 1.00
}{\aphistoxf}
\pgfplotstableread{
q vlad asmksp delfasmksp hqesp delfhqesp vggoffrmac resoffgem resftgem resftgemdfs resftgemspdfs
50 0.48 0.59 0.75 0.76 0.78 0.63 0.65 0.69 0.92 0.93
}{\aphistpar}


==> fig/data/ap_hist_q51.tex <==
\pgfplotstableread{
q vlad asmksp delfasmksp hqesp delfhqesp vggoffrmac resoffgem resftgem resftgemdfs resftgemspdfs
51 0.41 0.54 0.78 0.40 0.87 0.56 0.69 0.72 0.74 0.88
}{\aphistoxf}
\pgfplotstableread{
q vlad asmksp delfasmksp hqesp delfhqesp vggoffrmac resoffgem resftgem resftgemdfs resftgemspdfs
51 0.37 0.62 0.78 0.69 0.85 0.67 0.64 0.83 0.95 0.95
}{\aphistpar}


==> fig/data/ap_hist_q52.tex <==
\pgfplotstableread{
q vlad asmksp delfasmksp hqesp delfhqesp vggoffrmac resoffgem resftgem resftgemdfs resftgemspdfs
52 0.41 0.72 0.82 0.79 0.88 0.67 0.75 0.76 0.80 0.86
}{\aphistoxf}
\pgfplotstableread{
q vlad asmksp delfasmksp hqesp delfhqesp vggoffrmac resoffgem resftgem resftgemdfs resftgemspdfs
52 0.08 0.23 0.76 0.20 0.86 0.73 0.69 0.82 0.92 0.92
}{\aphistpar}


==> fig/data/ap_hist_q53.tex <==
\pgfplotstableread{
q vlad asmksp delfasmksp hqesp delfhqesp vggoffrmac resoffgem resftgem resftgemdfs resftgemspdfs
53 0.38 0.65 0.78 0.68 0.87 0.55 0.69 0.71 0.74 0.88
}{\aphistoxf}
\pgfplotstableread{
q vlad asmksp delfasmksp hqesp delfhqesp vggoffrmac resoffgem resftgem resftgemdfs resftgemspdfs
53 0.49 0.70 0.82 0.73 0.87 0.75 0.72 0.85 0.95 0.95
}{\aphistpar}


==> fig/data/ap_hist_q54.tex <==
\pgfplotstableread{
q vlad asmksp delfasmksp hqesp delfhqesp vggoffrmac resoffgem resftgem resftgemdfs resftgemspdfs
54 0.29 0.58 0.78 0.71 0.87 0.64 0.74 0.72 0.81 0.89
}{\aphistoxf}
\pgfplotstableread{
q vlad asmksp delfasmksp hqesp delfhqesp vggoffrmac resoffgem resftgem resftgemdfs resftgemspdfs
54 0.12 0.26 0.66 0.23 0.83 0.70 0.69 0.81 0.92 0.92
}{\aphistpar}


==> fig/data/ap_hist_q55.tex <==
\pgfplotstableread{
q vlad asmksp delfasmksp hqesp delfhqesp vggoffrmac resoffgem resftgem resftgemdfs resftgemspdfs
55 0.23 0.61 0.77 0.66 0.87 0.42 0.67 0.65 0.74 0.87
}{\aphistoxf}
\pgfplotstableread{
q vlad asmksp delfasmksp hqesp delfhqesp vggoffrmac resoffgem resftgem resftgemdfs resftgemspdfs
55 0.45 0.71 0.79 0.74 0.87 0.70 0.65 0.85 0.95 0.95
}{\aphistpar}


==> fig/data/ap_hist_q56.tex <==
\pgfplotstableread{
q vlad asmksp delfasmksp hqesp delfhqesp vggoffrmac resoffgem resftgem resftgemdfs resftgemspdfs
56 0.00 0.23 0.39 0.54 0.45 0.02 0.00 0.27 0.75 0.76
}{\aphistoxf}
\pgfplotstableread{
q vlad asmksp delfasmksp hqesp delfhqesp vggoffrmac resoffgem resftgem resftgemdfs resftgemspdfs
56 0.01 0.01 0.05 0.02 0.03 0.06 0.04 0.11 0.80 0.16
}{\aphistpar}


==> fig/data/ap_hist_q57.tex <==
\pgfplotstableread{
q vlad asmksp delfasmksp hqesp delfhqesp vggoffrmac resoffgem resftgem resftgemdfs resftgemspdfs
57 0.04 0.30 0.17 0.56 0.23 0.00 0.00 0.00 0.00 0.83
}{\aphistoxf}
\pgfplotstableread{
q vlad asmksp delfasmksp hqesp delfhqesp vggoffrmac resoffgem resftgem resftgemdfs resftgemspdfs
57 0.01 0.06 0.05 0.07 0.05 0.02 0.20 0.09 0.61 0.68
}{\aphistpar}


==> fig/data/ap_hist_q58.tex <==
\pgfplotstableread{
q vlad asmksp delfasmksp hqesp delfhqesp vggoffrmac resoffgem resftgem resftgemdfs resftgemspdfs
58 0.05 0.42 0.44 0.61 0.59 0.03 0.02 0.23 0.67 0.79
}{\aphistoxf}
\pgfplotstableread{
q vlad asmksp delfasmksp hqesp delfhqesp vggoffrmac resoffgem resftgem resftgemdfs resftgemspdfs
58 0.00 0.03 0.41 0.01 0.67 0.20 0.26 0.19 0.77 0.83
}{\aphistpar}


==> fig/data/ap_hist_q59.tex <==
\pgfplotstableread{
q vlad asmksp delfasmksp hqesp delfhqesp vggoffrmac resoffgem resftgem resftgemdfs resftgemspdfs
59 0.00 0.01 0.00 0.00 0.00 0.00 0.01 0.11 0.36 0.10
}{\aphistoxf}
\pgfplotstableread{
q vlad asmksp delfasmksp hqesp delfhqesp vggoffrmac resoffgem resftgem resftgemdfs resftgemspdfs
59 0.00 0.00 0.20 0.00 0.70 0.20 0.24 0.48 0.82 0.00
}{\aphistpar}


==> fig/data/ap_hist_q6.tex <==
\pgfplotstableread{
q vlad asmksp delfasmksp hqesp delfhqesp vggoffrmac resoffgem resftgem resftgemdfs resftgemspdfs
6 0.00 0.36 0.47 0.42 0.36 0.04 0.14 0.38 0.74 0.78
}{\aphistoxf}
\pgfplotstableread{
q vlad asmksp delfasmksp hqesp delfhqesp vggoffrmac resoffgem resftgem resftgemdfs resftgemspdfs
6 0.04 0.30 0.56 0.25 0.59 0.40 0.47 0.55 0.80 0.81
}{\aphistpar}


==> fig/data/ap_hist_q60.tex <==
\pgfplotstableread{
q vlad asmksp delfasmksp hqesp delfhqesp vggoffrmac resoffgem resftgem resftgemdfs resftgemspdfs
60 0.00 0.13 0.20 0.13 0.21 0.01 0.00 0.22 0.71 0.76
}{\aphistoxf}
\pgfplotstableread{
q vlad asmksp delfasmksp hqesp delfhqesp vggoffrmac resoffgem resftgem resftgemdfs resftgemspdfs
60 0.00 0.01 0.19 0.03 0.25 0.15 0.24 0.16 0.84 0.85
}{\aphistpar}


==> fig/data/ap_hist_q61.tex <==
\pgfplotstableread{
q vlad asmksp delfasmksp hqesp delfhqesp vggoffrmac resoffgem resftgem resftgemdfs resftgemspdfs
61 0.00 0.00 0.01 0.00 0.02 0.00 0.00 0.13 0.42 0.00
}{\aphistoxf}
\pgfplotstableread{
q vlad asmksp delfasmksp hqesp delfhqesp vggoffrmac resoffgem resftgem resftgemdfs resftgemspdfs
61 0.02 0.02 0.13 0.02 0.21 0.15 0.18 0.30 0.77 0.77
}{\aphistpar}


==> fig/data/ap_hist_q62.tex <==
\pgfplotstableread{
q vlad asmksp delfasmksp hqesp delfhqesp vggoffrmac resoffgem resftgem resftgemdfs resftgemspdfs
62 0.00 0.16 0.15 0.34 0.17 0.01 0.01 0.03 0.06 0.63
}{\aphistoxf}
\pgfplotstableread{
q vlad asmksp delfasmksp hqesp delfhqesp vggoffrmac resoffgem resftgem resftgemdfs resftgemspdfs
62 0.01 0.30 0.60 0.74 0.80 0.01 0.03 0.47 0.89 0.92
}{\aphistpar}


==> fig/data/ap_hist_q63.tex <==
\pgfplotstableread{
q vlad asmksp delfasmksp hqesp delfhqesp vggoffrmac resoffgem resftgem resftgemdfs resftgemspdfs
63 0.02 0.07 0.20 0.01 0.30 0.06 0.09 0.16 0.70 0.71
}{\aphistoxf}
\pgfplotstableread{
q vlad asmksp delfasmksp hqesp delfhqesp vggoffrmac resoffgem resftgem resftgemdfs resftgemspdfs
63 0.04 0.66 0.36 0.75 0.20 0.03 0.05 0.04 0.42 0.94
}{\aphistpar}


==> fig/data/ap_hist_q64.tex <==
\pgfplotstableread{
q vlad asmksp delfasmksp hqesp delfhqesp vggoffrmac resoffgem resftgem resftgemdfs resftgemspdfs
64 0.01 0.26 0.49 0.35 0.77 0.05 0.01 0.01 0.01 0.69
}{\aphistoxf}
\pgfplotstableread{
q vlad asmksp delfasmksp hqesp delfhqesp vggoffrmac resoffgem resftgem resftgemdfs resftgemspdfs
64 0.04 0.72 0.65 0.80 0.84 0.04 0.16 0.14 0.88 0.95
}{\aphistpar}


==> fig/data/ap_hist_q65.tex <==
\pgfplotstableread{
q vlad asmksp delfasmksp hqesp delfhqesp vggoffrmac resoffgem resftgem resftgemdfs resftgemspdfs
65 0.00 0.24 0.00 0.84 0.00 0.00 0.00 0.00 0.00 0.95
}{\aphistoxf}
\pgfplotstableread{
q vlad asmksp delfasmksp hqesp delfhqesp vggoffrmac resoffgem resftgem resftgemdfs resftgemspdfs
65 0.05 0.09 0.39 0.44 0.70 0.01 0.00 0.05 0.68 0.88
}{\aphistpar}


==> fig/data/ap_hist_q66.tex <==
\pgfplotstableread{
q vlad asmksp delfasmksp hqesp delfhqesp vggoffrmac resoffgem resftgem resftgemdfs resftgemspdfs
66 0.00 0.68 0.06 0.86 0.05 0.01 0.00 0.00 0.00 0.95
}{\aphistoxf}
\pgfplotstableread{
q vlad asmksp delfasmksp hqesp delfhqesp vggoffrmac resoffgem resftgem resftgemdfs resftgemspdfs
66 0.34 0.62 0.43 0.45 0.75 0.09 0.23 0.40 0.88 0.89
}{\aphistpar}


==> fig/data/ap_hist_q67.tex <==
\pgfplotstableread{
q vlad asmksp delfasmksp hqesp delfhqesp vggoffrmac resoffgem resftgem resftgemdfs resftgemspdfs
67 0.00 0.34 0.00 0.85 0.00 0.00 0.00 0.00 0.00 0.96
}{\aphistoxf}
\pgfplotstableread{
q vlad asmksp delfasmksp hqesp delfhqesp vggoffrmac resoffgem resftgem resftgemdfs resftgemspdfs
67 0.11 0.67 0.38 0.82 0.61 0.06 0.09 0.13 0.92 0.96
}{\aphistpar}


==> fig/data/ap_hist_q68.tex <==
\pgfplotstableread{
q vlad asmksp delfasmksp hqesp delfhqesp vggoffrmac resoffgem resftgem resftgemdfs resftgemspdfs
68 0.00 0.03 0.55 0.40 0.86 0.01 0.00 0.39 0.33 0.77
}{\aphistoxf}
\pgfplotstableread{
q vlad asmksp delfasmksp hqesp delfhqesp vggoffrmac resoffgem resftgem resftgemdfs resftgemspdfs
68 0.06 0.43 0.10 0.61 0.39 0.06 0.06 0.09 0.47 0.86
}{\aphistpar}


==> fig/data/ap_hist_q69.tex <==
\pgfplotstableread{
q vlad asmksp delfasmksp hqesp delfhqesp vggoffrmac resoffgem resftgem resftgemdfs resftgemspdfs
69 0.01 0.30 0.36 0.05 0.48 0.01 0.02 0.05 0.71 0.89
}{\aphistoxf}
\pgfplotstableread{
q vlad asmksp delfasmksp hqesp delfhqesp vggoffrmac resoffgem resftgem resftgemdfs resftgemspdfs
69 0.01 0.12 0.10 0.48 0.11 0.03 0.18 0.34 0.50 0.79
}{\aphistpar}


==> fig/data/ap_hist_q7.tex <==
\pgfplotstableread{
q vlad asmksp delfasmksp hqesp delfhqesp vggoffrmac resoffgem resftgem resftgemdfs resftgemspdfs
7 0.22 0.57 0.36 0.55 0.41 0.26 0.29 0.35 0.72 0.75
}{\aphistoxf}
\pgfplotstableread{
q vlad asmksp delfasmksp hqesp delfhqesp vggoffrmac resoffgem resftgem resftgemdfs resftgemspdfs
7 0.14 0.29 0.64 0.40 0.66 0.42 0.52 0.56 0.81 0.82
}{\aphistpar}


==> fig/data/ap_hist_q70.tex <==
\pgfplotstableread{
q vlad asmksp delfasmksp hqesp delfhqesp vggoffrmac resoffgem resftgem resftgemdfs resftgemspdfs
70 0.00 0.01 0.33 0.00 0.80 0.01 0.01 0.03 0.62 0.58
}{\aphistoxf}
\pgfplotstableread{
q vlad asmksp delfasmksp hqesp delfhqesp vggoffrmac resoffgem resftgem resftgemdfs resftgemspdfs
70 0.00 0.05 0.07 0.07 0.05 0.00 0.05 0.09 0.45 0.73
}{\aphistpar}


==> fig/data/ap_hist_q8.tex <==
\pgfplotstableread{
q vlad asmksp delfasmksp hqesp delfhqesp vggoffrmac resoffgem resftgem resftgemdfs resftgemspdfs
8 0.05 0.27 0.33 0.52 0.38 0.20 0.02 0.48 0.73 0.65
}{\aphistoxf}
\pgfplotstableread{
q vlad asmksp delfasmksp hqesp delfhqesp vggoffrmac resoffgem resftgem resftgemdfs resftgemspdfs
8 0.02 0.16 0.60 0.32 0.66 0.41 0.45 0.59 0.81 0.82
}{\aphistpar}


==> fig/data/ap_hist_q9.tex <==
\pgfplotstableread{
q vlad asmksp delfasmksp hqesp delfhqesp vggoffrmac resoffgem resftgem resftgemdfs resftgemspdfs
9 0.14 0.42 0.43 0.18 0.19 0.17 0.28 0.46 0.75 0.78
}{\aphistoxf}
\pgfplotstableread{
q vlad asmksp delfasmksp hqesp delfhqesp vggoffrmac resoffgem resftgem resftgemdfs resftgemspdfs
9 0.03 0.25 0.57 0.25 0.61 0.40 0.51 0.60 0.80 0.80
}{\aphistpar}


==> fig_split_groups.tex <==
\begin{figure}

\begin{center}
\foreach \q in {11,...,15}
{\includegraphics[height=1cm]{fig/oxford5k_queries/q\q.jpg} }

\vspace{1mm}
\foreach \q in {21,...,25}
{\includegraphics[height=1cm]{fig/oxford5k_queries/q\q.jpg} }

\vspace{1mm}
\foreach \q in {51,...,55}
{\includegraphics[height=1cm]{fig/paris6k_queries/q\q.jpg} }

\end{center}

\caption{Oxford and Paris original landmarks that were split in two groups.
\label{fig:split_groups}}

\end{figure}

==> tab_map_o100k_vs_r100k.tex <==
\newcolumntype{L}[1]{>{\raggedright\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
\newcolumntype{C}[1]{>{\centering\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
\newcolumntype{R}[1]{>{\raggedleft\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
\def\arraystretch{1.1}%  1 is the default, row height
\newcommand\cw{1.5cm}
% \centering
\footnotesize
% \setlength\extrarowheight{-1pt}
\begin{center}
\setlength{\tabcolsep}{0.2mm}
\begin{tabular}{|@{~}L{2cm}|C{\cw}|C{\cw}|C{\cw}|C{\cw}|}
    \hline
    \multirow{2}{*}{Method} & \multicolumn{2}{c|}{Medium} & \multicolumn{2}{c|}{Hard} \\
    \cline{2-5}
    & \roxf & \rpar & \roxf & \rpar \\
    \hline\hline
    \smk & 46.6 $\rightarrow$ (45.9)45.0 & 45.6 $\rightarrow$ (44.4)43.0 & 25.8 $\rightarrow$ (25.6)24.3 & 18.1 $\rightarrow$ (17.7)15.9 \\
    R--[O]--R-MAC & 40.3 $\rightarrow$ (37.9)32.7 & 63.1 $\rightarrow$ (61.5)59.4 & 9.9 $\rightarrow$ (9.8)5.5 & 36.6 $\rightarrow$ (34.7)32.9 \\
    R--\cite{RTC17}--GeM & 57.2 $\rightarrow$ (54.2)49.1 & 65.7 $\rightarrow$ (64.1)62.2 & 29.0 $\rightarrow$ (27.7)22.8 & 39.2 $\rightarrow$ (37.5)36.0 \\
    \hline
\end{tabular}
\end{center}
